HiPrompt: Few-Shot Biomedical Knowledge Fusion via Hierarchy-Oriented Prompting

Medical decision-making processes can be enhanced by comprehensive biomedical knowledge bases, which require fusing knowledge graphs constructed from different sources via a uniform index system. The index system often organizes biomedical terms in a hierarchy to provide the aligned entities with fine-grained granularity. To address the challenge of scarce supervision in the biomedical knowledge fusion (BKF) task, researchers have proposed various unsupervised methods. However, these methods heavily rely on ad-hoc lexical and structural matching algorithms, which fail to capture the rich semantics conveyed by biomedical entities and terms. Recently, neural embedding models have proved effective in semantic-rich tasks, but they rely on sufficient labeled data to be adequately trained. To bridge the gap between the scarce-labeled BKF and neural embedding models, we propose HiPrompt, a supervision-efficient knowledge fusion framework that elicits the few-shot reasoning ability of large language models through hierarchy-oriented prompts. Empirical results on the collected KG-Hi-BKF benchmark datasets demonstrate the effectiveness of HiPrompt.

==> figures/SDKG_DzTaxo_edit_dist.tex <==
\begin{tikzpicture}[scale=1.0]
  \foreach \y [count=\n] in {
      {5,30,65,118},
      {11,19,16,10},
      {6,26,23,31},
      {61,113,75,26},
    } {
      % column labels
      \foreach \a [count=\i] in {{[0,16)},{[16,24)},{[24,32)},{[32,$\infty$)}} {
        \node[minimum size=6mm] at (\i,-5) {\a};
      }
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=blue!\x!white, minimum size=10mm, text=black,font=\large] at (\m,-\n) {\x};
      }
    }
  % row labels
  \foreach \a [count=\i] in {{[12,$\infty$)},{[4,12)},{[1,4)},{[0,1)}} {
    \node[rotate=90,minimum size=6mm] at (0,-\i) {\a};
  }
  % x-axis label
  \node at (2.5,-5.5) {Avg. len. of entity names};
  % y-axis label
  \node [rotate=90] at (-0.5,-2.5) {Edit dist. between entity names};
\end{tikzpicture}

==> figures/benchmark_histo.tex <==
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
        group name=my plots,
        group size=1 by 2,
        xlabels at=edge bottom,
        xticklabels at=edge bottom,
        vertical sep=0pt
        },
        width  = 0.8\linewidth,
        ybar,
        axis lines*=left,
        ymajorgrids = true,
        ylabel = {Percentage (\%)},
        symbolic x coords={0,1-3,4-7,7-10,11-inf},
        xtick = data,
        scaled y ticks = false,
        %enlarge x limits=0.25,
        ymin=0,
        legend cell align=left,
        nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
        nodes near coords style={font=\scriptsize},
        every axis plot/.append style={fill},
        cycle list/Paired,
    ]
        \nextgroupplot[ymax=60]
        %SDKG-DzTaxo
        \addplot coordinates {(0, 39.17) (1-3,14.96) (4-7,4.42) (7-10,3.13) (11-inf, 38.32)};
        \nextgroupplot[ymax=60]
        %repoDB-DzTaxo
        \addplot coordinates {(0, 54.97) (1-3,6.94) (4-7,2.86) (7-10,8.57) (11-inf, 26.67)};
    \end{groupplot}
\end{tikzpicture}

==> figures/non_leaf_concepts_dist.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width  = \linewidth,
        ybar stacked,
        ymin = 0,
        axis lines*=left,
        ymajorgrids = true,
        ylabel = {Percentage (\%)},
        symbolic x coords={SDKG-DzTaxo,repoDB-DzTaxo},
        xtick = data,
        bar width=8mm,
        enlarge x limits=0.5,
        nodes near coords, 
        nodes near coords align={anchor=north},%Move values in bar
        every node near coord/.style={
        },
        %legend pos=outer north center,
        legend style={at={(0.5,-0.2)},anchor=north,legend columns=2},
    ]
    %leaf
    \addplot[style={fill=myblue1}]
        coordinates {(SDKG-DzTaxo, 86.77) (repoDB-DzTaxo,50.35)};
    %Non-leaf
    \addplot[style={fill=myorange1}]
        coordinates {(SDKG-DzTaxo,13.23) (repoDB-DzTaxo,49.65)};

    \legend{Leaf,Non-Leaf}
    \end{axis}
\end{tikzpicture}

==> figures/repoDB_DzTaxo_edit_dist.tex <==
\begin{tikzpicture}[scale=1.0]
  \foreach \y [count=\n] in {
      {5,70,61,32},
      {17,40,22,8},
      {18,22,6,4},
      {188,123,74,19},
    } {
      % column labels
      \foreach \a [count=\i] in {{[0,16)},{[16,24)},{[24,32)},{[32,$\infty$)}} {
        \node[minimum size=6mm] at (\i,-5) {\a};
      }
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=blue!\x!white, minimum size=10mm, text=black,font=\large] at (\m,-\n) {\x};
      }
    }
  % row labels
  \foreach \a [count=\i] in {{[12,$\infty$)},{[4,12)},{[1,4)},{[0,1)}} {
    \node[rotate=90,minimum size=6mm] at (0,-\i) {\a};
  }
  % x-axis label
  \node at (2.5,-5.5) {Avg. len. of entity names};
  % y-axis label
  \node [rotate=90] at (-0.5,-2.5) {Edit dist. between entity names};
\end{tikzpicture}

==> tables/neighbor_impact_archive.tex <==
\begin{table*}[htbp!]
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule
  \multicolumn{2}{c|}{HAKEGCN}&
  \multicolumn{2}{c|}{SEMedical $\times$ ReVerb} &
  \multicolumn{2}{c|}{SEMdical $\times$ OPIEC} &
  \multicolumn{2}{c|}{SEMusic $\times$ ReVerb} &
  \multicolumn{2}{c}{SEMusic $\times$ OPIEC} \\
$N_{CG}$ & $N_{OKG}$ & C-MRR & O-MRR & C-MRR & O-MRR & C-MRR & O-MRR & C-MRR & O-MRR \\ \hline
\checkmark &    &   .422&  .271&   .282&  .394&     .173& .118&       .380& .305\\
 & \checkmark &   .462&  .275& .532&  .412&   .435&  .178&      .543 & .421\\ 
\checkmark& \checkmark & .414& .273&    .363& .381&      .392 & .162&    .509&  .427\\
\bottomrule
\end{tabular}
\caption{neighbor impact on performance. $N_{CG}$ denotes whether to introduce taxonomic neighbors from Concept Graph, while $N_{OKG}$ denotes whether to introduce relational neighbors in Open Konlwedge Graph.}
\label{tab:neighbor_study}
\end{table*}
